Classification with neural networks with quadratic decision functions

Neural networks with quadratic decision functions have been introduced as alternatives to standard neural networks with affine linear ones. They are advantageous when the objects or classes to be identified are compact and of basic geometries like circles, ellipses etc. In this paper we investigate the use of such ansatz functions for classification. In particular we test and compare the algorithm on the MNIST dataset for classification of handwritten digits and for classification of subspecies. We also show, that the implementation can be based on the neural network structure in the software Tensorflow and Keras, respectively.

==> Makefile <==
MAIN = FriSchShi24

.PHONY: default full final clean check whoareyou bib help

default:
	pdflatex --file-line-error $(MAIN).tex

full:
	latexmk -pdf --file-line-error $(MAIN).tex

final:
	latexmk -pdf -interaction=nonstopmode --file-line-error -gg $(MAIN).tex
	biber --output_format=bibtex --output_resolve $(MAIN) -O biber.bib
	sed $(MAIN).tex -e '/^\\def\\notfinal{}/d' > $(MAIN)_final.tex
	latexmk -pdf -interaction=nonstopmode --file-line-error -gg $(MAIN)_final.tex
	latexmk -c $(MAIN).tex
	latexmk -c $(MAIN)_final.tex

clean:
	latexmk -c $(MAIN).tex
	rm -f $(MAIN).bbl $(MAIN).run.xml $(MAIN).thm $(MAIN).pdf

check:
	latexmk -pdf -interaction=nonstopmode --file-line-error -gg $(MAIN).tex

whoareyou:
	@echo $(MAIN)

bib:
	$(eval AUX := $(shell mktemp -d))
	latexmk -gg -pdf -jobname=extract -pdflatex="/usr/bin/pdflatex --file-line-error --shell-escape --synctex=1 %O '\def\extract{}\input{%S}'" -output-directory=${AUX} ${MAIN}.tex
	biber --output_format=bibtex --output_resolve -O ${AUX}/extract.bib ${AUX}/extract
	echo "\n%% Warning: This file is autogenerated, editing might be futile.\n" > csc.bib
	cat ${AUX}/extract.bib >> csc.bib

help:
	@echo ""
	@echo "make targets are:"
	@echo ""
	@echo "  default (default):"
	@echo "    just builds the tex file (without bibliography)"
	@echo ""
	@echo "  bib:"
	@echo "    extracts bibliography to csc.bib"
	@echo ""
	@echo "  full:"
	@echo "    builds the tex file (with bibliography)"
	@echo ""
	@echo "  final:"
	@echo "    extracts the bibliography into a local bib file"
	@echo "    creates an $(MAIN)_final.tex file using the extracted bib data"
	@echo ""
	@echo "  clean:"
	@echo "    cleans up temporary files"
	@echo ""
	@echo "  (check):"
	@echo "    used by the papercheck deamon, same as full but doesn't halt on error"
	@echo ""
	@echo "  (whoareyou):"
	@echo "    used by the papercheck daemon to identify this Makefile"
	@echo ""


